Citizens at the forefront of the constitutional debate: Participation determinants and emergent content in Chile

In the past few decades, constitution-making processes have shifted from closed elite writing to incorporating democratic mechanisms. Yet, little is known about democratic participation in deliberative constitution-making processes. Here, we study a deliberative constituent process held by the Chilean government between 2015 and 2016. The Chilean process had the highest level of citizen participation in the world ($204,402$ people, i.e., $1.3\%$ of the population) for such a process and covered $98\%$ of the national territory. In its participatory phase, people gathered in self-convoked groups of 10 to 30 members, and they collectively selected, deliberated, and wrote down an argument on why the new constitution should include those social rights. To understand the citizen participation drivers in this volunteer process, we first identify the determinants at the municipality level. We find the educational level, engagement in politics, support for the (left-wing) government, and Internet access increased participation. In contrast, population density and the share of evangelical Christians decreased participation. Moreover, we do not find evidence of political manipulation on citizen participation. In light of those determinants, we analyze the collective selection of social rights, and the content produced during the deliberative phase. The findings suggest that the knowledge embedded in cities, proxied using education levels and main economic activity, facilitates deliberation about themes, concepts, and ideas. These results can inform the organization of new deliberative processes that involve voluntary citizen participation, from citizen consultations to constitution-making processes.

==> Tables/words_stm.tex <==
\begin{table}[h!]
\scriptsize
  \caption{Word sets for three topics. All the STM analysis has been performed with the original texts in Spanish.     The words shown here have been translated into English.} 
\begin{center}
\begin{tabular}{L{3cm} L{4cm} L{4cm}}
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Highest Probability &  Frequent and exclusive \\ 
\hline \\[-1.8ex] 
\\[-1.8ex] 
Topic : Life & be, right, violence, all, death, conception, abortion, protect, respect, any, existence, natural, moment, human, nobody, born, euthanasia, life, obligation  & be, violence, death, conception, abortion, moment, born, euthanasia, respect, considered, fist, die, grounds, sentence, gestation, mothers, start, take off, pregnancy, fetus \\
\hline \\[-1.8ex] 
Topic: Environment & must, environment, resources, nature, natural, children, have, water, contamination, free, generations, respect, use, preservation, parents, sustainable, teaching, preserve, protection   & environment, nature, natural, children, water, contamination, generations, padres, sustainable, futures, healthy, clean, 	sustainability, environmental, air, planet, ecosystem, fauna \\
\hline \\[-1.8ex] 
Topic: Social security & social, must, security, system, condition, have, pensions, guarantee, economic, higher, disability, matter, age, decent, economic, old age, AFP$^{*}$, sexual, race   & social, condition, pensions, disability, age, old age, AFP, race, retirement, solidarity, pension, prevision, nationality, orientation, pay-as-you-go, color, 	unemployment \\
\hline \\[-1.8ex] 
\multicolumn{3}{p{12cm}}{\scriptsize{$^{*}$ The acronym AFP stands for \textit{ Administradoras de Fondos de Pensiones} (Pension Fund Administrators), Chilean private entities that manage private pension funds through an individual defined-contribution-based system.}} 
\end{tabular}
\end{center}
  \label{tab:words_stm}
\end{table}
